Partitioning graphs into induced subgraphs

We study the Induced $H$ Partition problem from the parameterized complexity point of view. In the Induced $H$ Partition problem the task is to partition vertices of a graph $G$ into sets $V_1,V_2,\dots,V_n$ such that the graph $H$ is isomorphic to the subgraph of $G$ induced by each set $V_i$ for $i = 1,2,\dots,n.$ The pattern graph $H$ is fixed. For the parametrization we consider three distinct structural parameters of the graph $G$ - namely the tree-width, the neighborhood diversity, and the modular-width. For the parametrization by the neighborhood diversity we obtain an FPT algorithm for every graph $H.$ For the parametrization by the tree-width we obtain an FPT algorithm for every connected graph $H.$ Finally, for the parametrization by the modular-width we derive an FPT algorithm for every prime graph $H.$

==> src/npHardnessPartition.tex <==
\section{The hardness of the \InducedHPartition problem}

The special case of the \InducedHPartition problem is the \TrianglePartition problem. It is well-known that this problem is \NP-complete. This fact can be shown by a reduction from the \ThreeDMatching problem (a special case of hypergraph version of the \PerfectMatching problem)---see Figure~\ref{fig:3DMtoTrP}.

\begin{figure}
  \input{tikz/triangleCoverNPh.tikz}
  \caption{An edge gadget used for the reduction from the \ThreeDMatching problem to the \TrianglePartition problem in left. In the middle an unselected edge and finally a selected edge in the right.}\label{fig:3DMtoTrP}
\end{figure}

\begin{figure}
  \input{tikz/cliqueCoverNPh.tikz}
  \caption{An edge gadget used for the reduction from the \ThreeDMatching problem to the \InducedHPartition problem in left (just for a clique case i.e. $H\simeq K_k$ for some $k\ge 3$). In the middle an unselected edge and finally a selected edge in the right. The $K^{red}_{k-3}$ is associated with the red vertex and the $K^e_{k-3}$ is associated with the hyperedge $e.$}\label{fig:3DMtoIK_kP}
\end{figure}

\begin{prob}{\ThreeDMatching}
INPUT: & A hypergraph $\mathcal{H} = (V, \mathcal{E})$ with $3n$ vertices, the set $V$ is divided into three sets $R, G, B$ with $|R| = |G| = |B| = n$ and satisfying $\mathcal{E}\subseteq R\times G\times B.$\\
QUESTION: & Does $\mathcal{H}$ have a perfect matching? That is a set $\mathcal{F}\subseteq\mathcal{E}$ such that $e\cap f=\emptyset$ for every $e,f\in\mathcal{F}$ and $|\mathcal{F}| = n.$\\
\end{prob}
We refer to vertex sets $R,G,B$ as to \emph{red, green} and \emph{blue vertices}.
The \ThreeDMatching problem is well-known to be \NP-complete as it is the seventeenth Karp problem~\cite{KarpNP}.

The reduction usually uses the sets of vertices $R, G, B$ (this is also our case) and a gadget $G_e$ for every hyperedge $e\in\mathcal{E}.$ However this is not sufficient for the general case---we have to extend this approach with several other gadgets. For example when the graph $H$ is isomorphic to $K_k$ (with $k\ge 3$) we have to add another copy extending also the red vertices---see Figure~\ref{fig:3DMtoIK_kP}.

\subsection{Having a triangle}
\paragraph{Decomposing $H$}
Let $H$ be fixed graph that contains a triangle ($K_3$) as a subgraph. We divide the vertices of the graph $H = (V, E)$ into four sets $V^T, V^{red},V^{green}, V^{blue}$ as follows. The set $V^T$ has exactly $3$ vertices and $H[V^T] \simeq K_3$ induces a fixed triangle---we refer to this as the triangle. We color the vertices of the triangle arbitrarily with colors red, green and blue. We may now slightly abuse the notation and write $V^T = \{r,g,b\}$ where we abbreviate red as $r$ and similarly for green and blue. The set $V^{red}$ contains vertices connected to the vertex $r,$ the set $V^{green}$ contains vertices connected to the vertex $g$ and finally the set $V^{blue}$ contains vertices connected to the vertex $b.$ We resolve ties arbitrarily to obtain $V^{c}\cap V^{d}=\emptyset$ for any distinct colors $c,d\in\{red, green, blue\}.$ To obtain a complete splitting of vertices of $H$ we add the remaining vertices (from the set $V\setminus(V^T\cup V^{red}\cup V^{green}\cup V^{blue})$) to sets $V^{red}, V^{green}, V^{blue}.$ Note that this may be done in a way that all graphs $H[V^{red}\cup\{r\}], H[V^{green}\cup\{g\}], H[V^{blue}\cup\{b\}]$ are connected (from connectedness of the graph $H$). For an example of a decomposition of the graph $H$ see Figure~\ref{fig:decompositionH}. We denote by $H^{red}$ the graph $H[V^{red}].$

\begin{figure}
  \begin{minipage}[c]{0.27\textwidth}
    \input{tikz/decompositionH.tikz}
  \end{minipage}
  \begin{minipage}[b]{0.72\textwidth}
    \caption{An example of a decomposition of a graph $H$ used in the \NP-hardness reduction.}
    \label{fig:decompositionH}
  \end{minipage}
\end{figure}

%Furthermore, we denote by $V^*$ the set of non-triangle vertices i.e. $V^* = V\setminus V^T = V^{red}\cup V^{green}\cup V^{blue}.$

\paragraph{The gadget}
The edge gadget we use for the reduction from the \ThreeDMatching problem is a generalization of the gadget from Figure~\ref{fig:3DMtoTrP}. We begin by identifying the triangle of $H$ (formed by vertices $r,g,b$) with the edge gadget triangle (vertices $1,2,3$ on figures). The vertex $r$ is mapped to the vertex $3,$ the vertex $g$ is mapped to the vertex $2$ and the vertex $b$ is mapped to the vertex $1.$

We follow the description with the part of the gadget for the vertices in set $V^{red}$---as it works similarly for all the other colors. As a basis for our gadget we took the gadget from Figure~\ref{fig:3DMtoTrP} (the left part). We now extend the gadget by adding a copy of the red part of the graph $H$ that is $H^{red}.$ It remains to add all the edges from the set $\delta(V^{red})$ to the gadget. If an edge $e \in\delta(V^{red})$ connects a vertex from the set $V^{red}$ to a vertex from the set $V^{green}$ we add it between the appropriate edge parts of the edge gadget and similarly with $V^{blue}.$

\paragraph{Extending the colored vertices}
Finally we have to add a graph $H^{red}$ to every red vertex in the constructed graph. The construction is essentially the same as for the edge but now the triangle is associated with the appropriate red vertex and vertices $1,2$ (in the case of $H^{green}$ and $H^{blue}$ the triangle is formed by the green vertex, the blue vertex and by the vertex $3.$). Here the numbered vertices are from all edge gadget containing the red vertex (the pair green and blue).

\paragraph{Verification of the construction}
It is easy to see that if the hypergraph $\mathcal{H}$ contains a perfect matching then it is possible to partition the constructed graph into copies of the given graph $H.$

For the other direction observe first, that without loss of generality we may assume that $V^{red}\neq\emptyset$ (if not we are left with the \TrianglePartition problem).

Now observe that if it is possible to partition the constructed graph $G$ into copies of $H$ the graph $H^{red}$ associated with a red vertex has to be used. It is impossible to use it without using the associated red vertex and vertices $1,2$ from the same edge (as the other vertices does not form a triangle in the graph $G$).
So the red vertex and the associated graph $H^{red}$ have to be further paired with $H^{green},H^{blue}$ from the edge containing the vertices $1,2$ (if any of these is nonempty).

Now it is easy to see that the only way how to finish the partition of $G$ is that the graphs $H^{green}, H^{blue}$ associated to the green and the blue vertices are used in a copy with the (only missing) graph $H^{red}$ form the edge gadget. This finishes our proof as such edges form a perfect matching in $\mathcal{H}.$

As this proof is rather technical, we encourage the reader to follow Figure~\ref{fig:3DMtoIK_kP} where $H\simeq K_k$ for the sake of simplicity---so $V^{red}$ is the only non-empty part in the decomposition of $H.$


